Identification and Estimation of Production Function with Unobserved Heterogeneity

This paper examines the nonparametric identifiability of production functions, considering firm heterogeneity beyond Hicks-neutral technology terms. We propose a finite mixture model to account for unobserved heterogeneity in production technology and productivity growth processes. Our analysis demonstrates that the production function for each latent type can be nonparametrically identified using four periods of panel data, relying on assumptions similar to those employed in existing literature on production function and panel data identification. By analyzing Japanese plant-level panel data, we uncover significant disparities in estimated input elasticities and productivity growth processes among latent types within narrowly defined industries. We further show that neglecting unobserved heterogeneity in input elasticities may lead to substantial and systematic bias in the estimation of productivity growth.

==> Output/Results_230421_initdraws=10_outlier_replaced/bias1_2223.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 08:46:50 2023
\begin{table}[ht]
\centering
\caption{Bias in $\Delta\tilde\omega$} 
\begin{tabular}{c|ccc}
  \hline
  & \multicolumn{3}{c}{J = 6} \\
 & Type 1 - 2& Type 3 - 4& Type 5 - 6 \\
 \hline
$\frac{\text{Mean of } |\text{Bias}_{it}|}{\text{Mean of }
                     |\Delta\tilde\omega_{it}|}$ & 0.098 & 0.104 & 0.099 \\ 
   \hline
$\beta_m^j$ & 0.287 & 0.326 & 0.394 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/bias1_2814.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 07:12:34 2023
\begin{table}[ht]
\centering
\caption{Bias in $\Delta\tilde\omega$} 
\begin{tabular}{c|ccc}
  \hline
  & \multicolumn{3}{c}{J = 6} \\
 & Type 1 - 2& Type 3 - 4& Type 5 - 6 \\
 \hline
$\frac{\text{Mean of } |\text{Bias}_{it}|}{\text{Mean of }
                     |\Delta\tilde\omega_{it}|}$ & 0.230 & 0.229 & 0.350 \\ 
   \hline
$\beta_m^j$ & 0.135 & 0.430 & 0.536 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/bias2_2223.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 08:46:50 2023
\begin{table}[ht]
\centering
\caption{Bias in $\Delta\tilde\omega$} 
\begin{tabular}{c|ccc}
  \hline
  & \multicolumn{3}{c}{J = 6} \\
 & Type 1 - 2& Type 3 - 4& Type 5 - 6 \\
 \hline
$\frac{\text{Mean of } \text{Bias}_{it}}
                  {\text{Mean of } |\Delta\tilde\omega_{it}|}
                  \Big|_{\Delta\omega_{it}>0}$ & -0.080 & -0.025 & 0.089 \\ 
   \hline
$\beta_m^j$ & 0.287 & 0.326 & 0.394 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/bias2_2814.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 07:12:34 2023
\begin{table}[ht]
\centering
\caption{Bias in $\Delta\tilde\omega$} 
\begin{tabular}{c|ccc}
  \hline
  & \multicolumn{3}{c}{J = 6} \\
 & Type 1 - 2& Type 3 - 4& Type 5 - 6 \\
 \hline
$\frac{\text{Mean of } \text{Bias}_{it}}
                  {\text{Mean of } |\Delta\tilde\omega_{it}|}
                  \Big|_{\Delta\omega_{it}>0}$ & -0.201 & 0.156 & 0.203 \\ 
   \hline
$\beta_m^j$ & 0.135 & 0.430 & 0.536 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/distprod_2223.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 08:46:50 2023
\begin{table}[ht]
\centering
\caption{Standard Deviations of $\omega_{it}$ and $\epsilon_{it}$} 
\begin{tabular}{c|c|ccccccc}
  \hline
  & J = 1 & \multicolumn{7}{c}{J = 6} \\
 & & Type 1& Type 2& Type 3& Type 4& Type 5& Type 6 & Ave \\
 \hline
%Std. Dev. $\hat\omega_{it}+\beta_{\ell}^j\psi^j + \beta_{0t}^j$ & 0.432 & 0.257 & 0.226 & 0.672 & 0.487 & 0.203 & 0.237 & 0.281 \\ 
  Std. Dev. $\hat\omega_{it} + \beta_{0t}^j$ & 0.432 & 0.257 & 0.226 & 0.672 & 0.487 & 0.203 & 0.237 & 0.281 \\ 
  Std. Dev. $\hat\epsilon_{it}$ & 0.350 & 0.340 & 0.303 & 0.416 & 0.401 & 0.274 & 0.254 & 0.312 \\ 
  $Corr(\hat\epsilon_{it},\hat\epsilon_{it-1})$ & 0.812 & 0.792 & 0.764 & 0.752 & 0.779 & 0.747 & 0.736 & 0.761 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/distprod_2814.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 07:12:33 2023
\begin{table}[ht]
\centering
\caption{Standard Deviations of $\omega_{it}$ and $\epsilon_{it}$} 
\begin{tabular}{c|c|ccccccc}
  \hline
  & J = 1 & \multicolumn{7}{c}{J = 6} \\
 & & Type 1& Type 2& Type 3& Type 4& Type 5& Type 6 & Ave \\
 \hline
%Std. Dev. $\hat\omega_{it}+\beta_{\ell}^j\psi^j + \beta_{0t}^j$ & 1.387 & 0.832 & 0.661 & 0.735 & 0.505 & 0.347 & 0.338 & 0.612 \\ 
  Std. Dev. $\hat\omega_{it} + \beta_{0t}^j$ & 1.387 & 0.832 & 0.661 & 0.735 & 0.505 & 0.347 & 0.338 & 0.612 \\ 
  Std. Dev. $\hat\epsilon_{it}$ & 0.792 & 0.694 & 0.462 & 0.655 & 0.311 & 0.253 & 0.233 & 0.479 \\ 
  $Corr(\hat\epsilon_{it},\hat\epsilon_{it-1})$ & 0.883 & 0.737 & 0.670 & 0.661 & 0.686 & 0.709 & 0.761 & 0.710 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/parameters_2223.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 08:46:40 2023
\begin{table}[ht]
\centering
\caption{Estimates of Production Function} 
\begin{tabular}{c|c|cccccc}
  \hline
  & J = 1 & \multicolumn{6}{c}{J = 6} \\
 & & Type 1& Type 2& Type 3& Type 4& Type 5& Type 6 \\
 \hline
$\beta_m^j$ & 0.332 & 0.287 & 0.287 & 0.326 & 0.326 & 0.394 & 0.394 \\ 
   & ( 0.004 ) &( 0.005 )&( 0.005 )&( 0.012 )&( 0.012 )&( 0.005 )&( 0.005 ) \\
$\beta_{\ell}^j$ & 0.224 & 0.263 & 0.263 & 0.220 & 0.220 & 0.186 & 0.186 \\ 
   & ( 0.003 ) &( 0.005 )&( 0.005 )&( 0.009 )&( 0.009 )&( 0.003 )&( 0.003 ) \\
$\beta_k^j$ & 0.075 & 0.147 & 0.147 & 0.172 & 0.172 & 0.103 & 0.103 \\ 
   & ( 0.015 ) &( 0.036 )&( 0.036 )&( 0.034 )&( 0.034 )&( 0.014 )&( 0.014 ) \\
 \hline
$\beta_m^j + \beta_{\ell}^j + \beta_k^j$ & 0.632 & 0.696 & 0.696 & 0.719 & 0.719 & 0.683 & 0.683 \\ 
  $\beta_k^j/\beta_{\ell}^j$ & 0.336 & 0.558 & 0.558 & 0.780 & 0.780 & 0.556 & 0.556 \\ 
  $\Sigma_{t=1}^T\beta_{0,t}^j/T$ & 6.218 & 5.604 & 5.604 & 5.303 & 5.303 & 5.449 & 5.449 \\ 
   \hline
$\psi^j$ & 0.000 & -0.108 & 0.344 & -1.454 & 0.534 & 0.056 & 0.627 \\ 
   & ( NA ) &( 0.086 )&( 0.090 )&( 0.339 )&( 0.081 )&( 0.085 )&( 0.088 ) \\
 \hline
$\pi$ & 1.000 & 0.174 & 0.240 & 0.051 & 0.119 & 0.263 & 0.152 \\ 
   & ( NA ) &( 0.014 )&( 0.019 )&( 0.015 )&( 0.021 )&( 0.018 )&( 0.015 ) \\\hline
 Obs & \multicolumn{7}{c}{13892} \\
 No. Plants & \multicolumn{7}{c}{914} \\
 \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/parameters_2814.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 07:12:26 2023
\begin{table}[ht]
\centering
\caption{Estimates of Production Function} 
\begin{tabular}{c|c|cccccc}
  \hline
  & J = 1 & \multicolumn{6}{c}{J = 6} \\
 & & Type 1& Type 2& Type 3& Type 4& Type 5& Type 6 \\
 \hline
$\beta_m^j$ & 0.281 & 0.135 & 0.135 & 0.430 & 0.430 & 0.536 & 0.536 \\ 
   & ( 0.008 ) &( 0.022 )&( 0.022 )&( 0.029 )&( 0.029 )&( 0.054 )&( 0.054 ) \\
$\beta_{\ell}^j$ & 0.296 & 0.496 & 0.496 & 0.163 & 0.163 & 0.195 & 0.195 \\ 
   & ( 0.006 ) &( 0.016 )&( 0.016 )&( 0.010 )&( 0.010 )&( 0.041 )&( 0.041 ) \\
$\beta_k^j$ & 0.076 & 0.146 & 0.146 & 0.186 & 0.186 & 0.175 & 0.175 \\ 
   & ( 0.016 ) &( 0.031 )&( 0.031 )&( 0.027 )&( 0.027 )&( 0.049 )&( 0.049 ) \\
 \hline
$\beta_m^j + \beta_{\ell}^j + \beta_k^j$ & 0.652 & 0.776 & 0.776 & 0.778 & 0.778 & 0.906 & 0.906 \\ 
  $\beta_k^j/\beta_{\ell}^j$ & 0.256 & 0.294 & 0.294 & 1.140 & 1.140 & 0.893 & 0.893 \\ 
  $\Sigma_{t=1}^T\beta_{0,t}^j/T$ & 6.125 & 5.747 & 5.747 & 4.560 & 4.560 & 2.992 & 2.992 \\ 
   \hline
$\psi^j$ & 0.000 & -1.084 & 0.452 & -0.551 & 1.178 & -0.534 & 0.540 \\ 
   & ( NA ) &( 0.249 )&( 0.080 )&( 0.062 )&( 0.109 )&( 0.390 )&( 0.146 ) \\
 \hline
$\pi$ & 1.000 & 0.278 & 0.168 & 0.163 & 0.098 & 0.109 & 0.184 \\ 
   & ( NA ) &( 0.033 )&( 0.046 )&( 0.015 )&( 0.044 )&( 0.027 )&( 0.022 ) \\\hline
 Obs & \multicolumn{7}{c}{10913} \\
 No. Plants & \multicolumn{7}{c}{907} \\
 \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/regIK_2223.tex <==

\begin{table}
\caption{The Effect of $\omega_{it}$ on Investment}
\begin{center}
\begin{tabular}{l c c c c c c c}
\hline
 & Single type & Type 1 & Type 2 & Type 3 & Type 4 & Type 5 & Type 6 \\
\hline
$\alpha^j_{\omega}$          & $0.059$   & $0.059$   & $0.061$   & $0.048$   & $-0.163$  & $0.076$   & $0.081$   \\
                             & $(0.024)$ & $(0.013)$ & $(0.014)$ & $(0.037)$ & $(0.140)$ & $(0.011)$ & $(0.011)$ \\
$\gamma^j_{\omega}(0.10)$    & $0.002$   & $0.004$   & $0.001$   & $-0.000$  & $0.014$   & $0.016$   & $0.018$   \\
                             & $(0.000)$ & $(0.003)$ & $(0.000)$ & $(0.004)$ & $(0.004)$ & $(0.003)$ & $(0.004)$ \\
$\gamma^j_{\omega}(0.25)$    & $0.007$   & $0.016$   & $0.011$   & $0.001$   & $0.010$   & $0.023$   & $0.029$   \\
                             & $(0.001)$ & $(0.003)$ & $(0.003)$ & $(0.003)$ & $(0.002)$ & $(0.003)$ & $(0.004)$ \\
$\gamma^j_{\omega}(0.50)$    & $0.017$   & $0.031$   & $0.031$   & $0.011$   & $0.022$   & $0.044$   & $0.040$   \\
                             & $(0.001)$ & $(0.005)$ & $(0.005)$ & $(0.006)$ & $(0.004)$ & $(0.005)$ & $(0.005)$ \\
$\gamma^j_{\omega}(0.75)$    & $0.037$   & $0.049$   & $0.065$   & $0.050$   & $0.030$   & $0.073$   & $0.080$   \\
                             & $(0.003)$ & $(0.009)$ & $(0.008)$ & $(0.016)$ & $(0.007)$ & $(0.008)$ & $(0.009)$ \\
$\gamma^j_{\omega}(0.90)$    & $0.072$   & $0.077$   & $0.125$   & $0.091$   & $0.025$   & $0.124$   & $0.110$   \\
                             & $(0.007)$ & $(0.025)$ & $(0.024)$ & $(0.021)$ & $(0.018)$ & $(0.025)$ & $(0.023)$ \\
\hline
$\beta_m^j$                  & $0.332$   & $0.287$   & $0.287$   & $0.326$   & $0.326$   & $0.394$   & $0.394$   \\
$\beta_k^j/\beta_{\ell}^j$   & $0.336$   & $0.558$   & $0.558$   & $0.780$   & $0.780$   & $0.556$   & $0.556$   \\
$\overline{(I_{it}/K_{it})}$ & $0.104$   & $0.080$   & $0.085$   & $0.141$   & $0.264$   & $0.075$   & $0.069$   \\
\hline
\end{tabular}
\label{table:coefficients}
\end{center}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/regIK_2814.tex <==

\begin{table}
\caption{The Effect of $\omega_{it}$ on Investment}
\begin{center}
\begin{tabular}{l c c c c c c c}
\hline
 & Single type & Type 1 & Type 2 & Type 3 & Type 4 & Type 5 & Type 6 \\
\hline
$\alpha^j_{\omega}$          & $0.500$   & $-0.215$  & $-0.113$  & $0.188$   & $0.171$   & $0.080$   & $0.079$   \\
                             & $(0.110)$ & $(0.138)$ & $(0.974)$ & $(0.401)$ & $(0.079)$ & $(0.020)$ & $(0.014)$ \\
$\gamma^j_{\omega}(0.10)$    & $0.002$   & $0.002$   & $-0.000$  & $0.002$   & $0.014$   & $0.004$   & $0.004$   \\
                             & $(0.000)$ & $(0.001)$ & $(0.000)$ & $(0.001)$ & $(0.006)$ & $(0.002)$ & $(0.003)$ \\
$\gamma^j_{\omega}(0.25)$    & $0.001$   & $0.000$   & $0.000$   & $0.000$   & $0.013$   & $0.006$   & $0.012$   \\
                             & $(0.000)$ & $(0.002)$ & $(0.003)$ & $(0.000)$ & $(0.004)$ & $(0.003)$ & $(0.003)$ \\
$\gamma^j_{\omega}(0.50)$    & $0.010$   & $0.003$   & $0.010$   & $0.010$   & $0.030$   & $0.030$   & $0.050$   \\
                             & $(0.001)$ & $(0.001)$ & $(0.003)$ & $(0.002)$ & $(0.006)$ & $(0.009)$ & $(0.005)$ \\
$\gamma^j_{\omega}(0.75)$    & $0.028$   & $0.016$   & $0.031$   & $0.039$   & $0.048$   & $0.071$   & $0.074$   \\
                             & $(0.002)$ & $(0.004)$ & $(0.006)$ & $(0.007)$ & $(0.011)$ & $(0.017)$ & $(0.011)$ \\
$\gamma^j_{\omega}(0.90)$    & $0.060$   & $0.011$   & $0.032$   & $0.097$   & $0.060$   & $0.115$   & $0.106$   \\
                             & $(0.004)$ & $(0.011)$ & $(0.014)$ & $(0.018)$ & $(0.015)$ & $(0.024)$ & $(0.028)$ \\
\hline
$\beta_m^j$                  & $0.281$   & $0.135$   & $0.135$   & $0.430$   & $0.430$   & $0.536$   & $0.536$   \\
$\beta_k^j/\beta_{\ell}^j$   & $0.256$   & $0.294$   & $0.294$   & $1.140$   & $1.140$   & $0.893$   & $0.893$   \\
$\overline{(I_{it}/K_{it})}$ & $0.335$   & $0.350$   & $0.828$   & $0.471$   & $0.165$   & $0.073$   & $0.079$   \\
\hline
\end{tabular}
\label{table:coefficients}
\end{center}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/sumstats_2223.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 07:21:58 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrr}
  \hline
 & n & mean & sd & min & max \\ 
  \hline
id & 13892 & 273366.31 & 259256.28 & 1397.00 & 1491177.00 \\ 
  year & 13892 & 1995.93 & 6.56 & 1986.00 & 2010.00 \\ 
  y\_it & 13892 & 11.37 & 0.68 & 7.60 & 14.39 \\ 
  lnmY\_it & 13892 & -0.98 & 0.35 & -1.83 & -0.33 \\ 
  l\_it & 13892 & 3.97 & 0.41 & 3.40 & 6.81 \\ 
  k\_it & 13892 & 10.91 & 0.86 & 5.22 & 14.06 \\ 
  m\_it & 13892 & 10.34 & 0.83 & -0.13 & 13.89 \\ 
  industry\_2 & 13892 & 2223.00 & 0.00 & 2223.00 & 2223.00 \\ 
  laborcost & 13892 & 23720.19 & 19463.26 & 331.00 & 395347.00 \\ 
  lnlY\_it & 13892 & -1.47 & 0.43 & -2.39 & -0.50 \\ 
  va & 13892 & 10.80 & 0.95 & 0.00 & 13.76 \\ 
  export & 13892 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  I\_K & 13892 & 0.10 & 1.06 & -1.04 & 115.02 \\ 
  flag\_main & 13892 & 1.00 & 0.00 & 1.00 & 1.00 \\ 
  flag\_size & 13892 & 1.00 & 0.00 & 1.00 & 1.00 \\ 
  flag\_IK\_data & 13892 & 0.96 & 0.20 & 0.00 & 1.00 \\ 
  icode\_2x & 13892 & 22.00 & 0.07 & 19.00 & 22.00 \\ 
  icode\_3x & 13892 & 222.00 & 0.00 & 222.00 & 222.00 \\ 
  icode\_4x & 13892 & 2223.00 & 0.00 & 2223.00 & 2223.00 \\ 
  t & 13892 & 1995.93 & 6.56 & 1986.00 & 2010.00 \\ 
  lc & 13892 & 9.91 & 0.53 & 5.80 & 12.89 \\ 
  l.lag & 12978 & 3.98 & 0.41 & 3.40 & 6.81 \\ 
  k.lag & 12978 & 10.92 & 0.86 & 5.30 & 14.06 \\ 
  m.lag & 12978 & 10.36 & 0.82 & -0.13 & 13.72 \\ 
  dum\_ex & 13892 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/sumstats_2814.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Fri Apr 21 06:45:58 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrr}
  \hline
 & n & mean & sd & min & max \\ 
  \hline
id & 10913 & 240761.23 & 293700.54 & 5142.00 & 1498109.00 \\ 
  year & 10913 & 1994.65 & 6.43 & 1986.00 & 2010.00 \\ 
  y\_it & 10913 & 11.24 & 1.78 & 5.51 & 17.35 \\ 
  lnmY\_it & 10913 & -0.99 & 0.79 & -3.13 & -0.08 \\ 
  l\_it & 10913 & 4.51 & 0.90 & 3.40 & 8.53 \\ 
  k\_it & 10913 & 10.04 & 1.99 & 1.67 & 16.22 \\ 
  m\_it & 10913 & 10.37 & 2.31 & 3.27 & 16.89 \\ 
  industry\_2 & 10913 & 2814.00 & 0.00 & 2814.00 & 2814.00 \\ 
  laborcost & 10913 & 68770.11 & 248254.01 & 261.00 & 17900000.00 \\ 
  lnlY\_it & 10913 & -1.39 & 0.78 & -3.11 & -0.16 \\ 
  va & 10913 & 10.59 & 1.76 & 0.00 & 16.65 \\ 
  export & 10913 & 0.96 & 6.82 & 0.00 & 98.20 \\ 
  I\_K & 10913 & 0.34 & 11.49 & -1.28 & 1030.83 \\ 
  flag\_main & 10913 & 1.00 & 0.00 & 1.00 & 1.00 \\ 
  flag\_size & 10913 & 1.00 & 0.00 & 1.00 & 1.00 \\ 
  flag\_IK\_data & 10913 & 0.94 & 0.24 & 0.00 & 1.00 \\ 
  icode\_2x & 10913 & 27.88 & 1.06 & 9.00 & 32.00 \\ 
  icode\_3x & 10913 & 280.89 & 4.72 & 193.00 & 329.00 \\ 
  icode\_4x & 10913 & 2814.00 & 0.00 & 2814.00 & 2814.00 \\ 
  t & 10913 & 1994.65 & 6.43 & 1986.00 & 2010.00 \\ 
  lc & 10913 & 10.09 & 1.20 & 5.56 & 16.70 \\ 
  l.lag & 10006 & 4.55 & 0.90 & 3.40 & 8.39 \\ 
  k.lag & 10006 & 10.08 & 1.99 & 1.67 & 16.22 \\ 
  m.lag & 10006 & 10.43 & 2.30 & 3.27 & 16.89 \\ 
  dum\_ex & 10913 & 0.04 & 0.18 & 0.00 & 1.00 \\ 
   \hline
\end{tabular}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/test_hetero_2223.tex <==

\begin{table}
\caption{A Test for Heterogeneity}
\begin{center}
\begin{tabular}{l c}
\hline
 & Model 1 \\
\hline
Intercept  & $0.0096^{***}$  \\
           & $(0.0012)$      \\
$m^2$      & $0.0083^{***}$  \\
           & $(0.0001)$      \\
$\ell^2$   & $0.0098^{***}$  \\
           & $(0.0007)$      \\
$k^2$      & $0.0014^{***}$  \\
           & $(0.0001)$      \\
$m\ell$    & $-0.0214^{***}$ \\
           & $(0.0004)$      \\
$\ell k$   & $0.0129^{***}$  \\
           & $(0.0005)$      \\
$km$       & $-0.0079^{***}$ \\
           & $(0.0003)$      \\
\hline
R$^2$      & $0.4470$        \\
Adj. R$^2$ & $0.4468$        \\
Num. obs.  & $13892$         \\
\hline
\multicolumn{2}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}
\label{table:coefficients}
\end{center}
\end{table}


==> Output/Results_230421_initdraws=10_outlier_replaced/test_hetero_2814.tex <==

\begin{table}
\caption{A Test for Heterogeneity}
\begin{center}
\begin{tabular}{l c}
\hline
 & Model 1 \\
\hline
Intercept  & $-0.0022^{*}$   \\
           & $(0.0009)$      \\
$m^2$      & $0.0009^{***}$  \\
           & $(0.0001)$      \\
$\ell^2$   & $0.0033^{***}$  \\
           & $(0.0006)$      \\
$k^2$      & $0.0008^{***}$  \\
           & $(0.0001)$      \\
$m\ell$    & $-0.0019^{***}$ \\
           & $(0.0004)$      \\
$\ell k$   & $-0.0011^{**}$  \\
           & $(0.0004)$      \\
$km$       & $-0.0008^{***}$ \\
           & $(0.0002)$      \\
\hline
R$^2$      & $0.0380$        \\
Adj. R$^2$ & $0.0374$        \\
Num. obs.  & $10913$         \\
\hline
\multicolumn{2}{l}{\scriptsize{$^{***}p<0.001$; $^{**}p<0.01$; $^{*}p<0.05$}}
\end{tabular}
\label{table:coefficients}
\end{center}
\end{table}

